Inference Trees: Adaptive Inference with Exploration

We introduce inference trees (ITs), a new class of inference methods that build on ideas from Monte Carlo tree search to perform adaptive sampling in a manner that balances exploration with exploitation, ensures consistency, and alleviates pathologies in existing adaptive methods. ITs adaptively sample from hierarchical partitions of the parameter space, while simultaneously learning these partitions in an online manner. This enables ITs to not only identify regions of high posterior mass, but also maintain uncertainty estimates to track regions where significant posterior mass may have been missed. ITs can be based on any inference method that provides a consistent estimate of the marginal likelihood. They are particularly effective when combined with sequential Monte Carlo, where they capture long-range dependencies and yield improvements beyond proposal adaptation alone.

==> combine.tex <==
% !TEX root =  it_icml2018.tex

To demonstrate how estimates can be combined from different partitions 
we consider the case of using importance sampling for the running 
inference locally . Let 
\begin{align}
\begin{split}
\label{eq:app:trun_prop}
Q\left(x_{1:T} \mid \{z_{1:T}\in B_i\}\right) & =
q_{i,1} (x_1 | \{z_1\in Z_{i,1} \}) \\ \prod_{t=2}^{T} &q_{i,t} (x_t | x_{1:t-1}, \{z_t\in Z_{i,t} \})
\end{split}
\end{align}
be the overall truncated proposal for region $B_i$.  We now have for marginal
likelihood estimation
\begin{align}
p(Y) 
& = \int \sum_{i \in \mathcal{I}} \iden(x_{1:T} \in A_i)p(x_{1:T}, Y)\, dx_{1:T}
 \nonumber
\\
%= &\sum_{i \in \mathcal{I}} \int \iden(z_{1:T} \in B_i)p(x_{1:T}, Y)\, dx_{1:T} \nonumber \\
 = &\sum_{i \in \mathcal{I}} \int p(x_{1:T}, Y)
\prod_{t=1}^T \iden(z_{t} \in Z_{i,t}) \, dx_{1:T} 
\nonumber
\\
= & \sum_{i \in \mathcal{I}} \expt_{Q\left(x_{1:T} \mid \{z_{1:T}\in B_i\}\right)} 
\left[\frac{ p(x_{1:T}, Y) \prod_{t=1}^T \iden(z_{t} \in Z_{i,t}) }
{Q\left(x_{1:T} \mid \{z_{1:T}\in B_i\}\right)}\right] 
\nonumber \\
\approx &\sum_{i \in \mathcal{I}} \hat{\upsilon}_i \quad \text{where each} \quad \hat{\upsilon}_i = \frac{1}{N_i}\sum_{n=1}^{N_i}
w_n^i, \nonumber \\
& w_n^i = \frac{ p(\hat{x}^n_{1:T,i}, Y) \prod_{t=1}^T \iden(\hat{z}_{t,i}^n \in
	 Z_{i,t}) }
{Q\left(\hat{x}^n_{1:T,i} \middle| \{\hat{z}_{1:T,i}^n\in B_i\}\right)},
\label{eq:ML-comb}
\end{align}
$\hat{x}^n_{1:T,i} \sim Q\left(x_{1:T} \mid \{z_{1:T}\in B_i\}\right)$,
and $\hat{z}_{1:T,i}^n$ is implied by $\hat{x}^n_{1:T,i}$.  Note here that each $\hat{\upsilon}_i$ is
an estimate of the marginal probability $p(\{z_{1:T} \in B_i\},Y) = p(\{x_{1:T} \in A_i\},Y)$.

If we instead consider the case of calculating an expectation we now have
\begin{align}
&\expt_{p(x_{1:T} |Y)} [f(x_{1:T})] 
=  \frac{1}{p(Y)} \int p(x_{1:T},Y) f(x_{1:T}) \, dx_{1:T}  \nonumber \\
&= \frac{1}{p(Y)}\sum_{i \in \mathcal{I}} \int p(x_{1:T}, Y) f(x_{1:T})
\prod_{t=1}^T \iden(z_{t} \in Z_{i,t}) \, dx_{1:T} \nonumber \\
&= \frac{1}{p(Y)} \sum_{i \in \mathcal{I}} \expt_{Q} %\left(x_{1:T} \mid \{z_{1:T}\in B_i\}\right)} 
\left[\frac{ p(x_{1:T}, Y) f(x_{1:T})\prod_{t=1}^T \iden(z_{t} \in Z_{i,t}) }
{Q\left(x_{1:T} \mid \{z_{1:T}\in B_i\}\right)}\right] \nonumber \\
&\approx \frac{\sum_{i \in \mathcal{I}} \hat{\varrho}_i}
{\sum_{i \in \mathcal{I}} \hat{\upsilon}_i } \quad \text{where} \quad
\hat{\varrho}_i = \frac{1}{N_i}\sum_{n=1}^{N_i}
w_n^i f\left(\hat{x}_{1:T,i}^n\right),
\label{eq:app:expt-comb}
\end{align}
each $\hat{\varrho}_i$ is an estimate of $\mu_i := \expt_{p(x_{1:T} |Y)} [f(x_{1:T}) p(Y) \iden(x_{1:T} \in A_i)]$ 
and the weights are defined as before.  Note that we are using self-normalization
for the importance sampling, but that we are doing this globally rather than
locally --  though the $w_n^i$ are not normalized, the normalization constant for all weights is 
the same  global constant $p(Y)$ (because the proposals are
correctly normalized within their target area).
In general, we will propagate \emph{unnormalized}
estimates $\hat{\varrho}_i$, only normalizing them at the root node using the marginal
probability estimates $\hat{\upsilon}_i$
which are themselves propagated through the tree separately.  Note that $f\left(x_{1:T}\right)=1, \; \forall x_{1:T} \in \X_T$ 
is a special case giving marginal likelihood estimates, so we can use the same approaches 
for $\hat{\upsilon}_i$ as for $\hat{\varrho}_i$.  Namely, analogously to~$\hat{\mu}_j$, we
define $\hat{\omega}_j=\hat{\upsilon}_i$ for the leaf nodes and for the others
\begin{align}
\label{eq:estimate-W}
%\begin{split}
%& \hat{\mu}_j(x_{1:T}, Y , \{z_{1:T}  \in B_j\}) = 
%\frac{c_j-\left(c_{l_j}+c_{r_j}\right)}{c_j} \hat{\varrho}_j(x_{1:T})
%\\
%&
%\qquad
%{}+\frac{c_{l_j}+c_{r_j}}{c_j} \left( \hat{\mu}_{l_j}(x_{1:T}, Y, \{z_{1:T}  \in B_j\}) +  \hat{\mu}_{r_j}(x_{1:T}, Y,  \{z_{1:T}  \in B_j\})\right).
%\end{split}
\hat{\omega}_j = 
\frac{c_j-\left(c_{l_j}+c_{r_j}\right)}{c_j} \hat{\upsilon}_j
+\frac{c_{l_j}+c_{r_j}}{c_j} \left( \hat{\omega}_{l_j}+  \hat{\omega}_{r_j}\right).
\end{align}

We can calculate a Monte Carlo empirical measure approximation for 
the posterior using the same approach as $\hat{\varrho}_j$, namely
\begin{align}
p(x_{1:T} | Y) \approx \frac{\sum_{i \in \mathcal{I}} \frac{1}{N_i}\sum_{n=1}^{N_i}
	w_n^i \delta_{\hat{x}_{1:T,i}^n} (x_{1:T})}
{\sum_{i \in \mathcal{I}} \hat{\upsilon}_i }.
\label{eq:post-comb:app}
\end{align}
Note that we are combining estimates from different partitions in an unweighted manner --
there is no need to apply correction factors for the strategy used to
assign computational resources.  We can do this because the weights are calculated using 
correctly normalized proposal distributions as per~\eqref{eq:prop}.

Using SMC inference at each of the nodes follows the same derivation with the weights
appropriately redefined (namely they are the product of the marginal likelihood estimate and
the local self-normalized weight from the sweep).  For notational consistency later
in the tree training algorithm,
will use $n$ to index an SMC sweep, rather than individual sample, such that 
each $\hat{x}_{1:T,i}^n$ and $w_n^i$ itself corresponds to a set of particles and corresponding weights.

More generally, we can use any method for which each
$\hat{\varrho}_i$ and $\hat{\upsilon}_i$ are consistent estimates
as $N_i\to \infty$.  An important consequence of this is that we can use ITs in
pseudo-marginal~\cite{andrieu2009pseudo} situations when the likelihood cannot
be directly evaluated but can be estimated unbiasedly.  This means that, for example,
we can run SMC where there as some latent variables not directly control by the IT
algorithm, i.e. $p(x_{1:T} | Y) = \int p(x_{1:T},u_{1:S} | Y) du_{1:S}$ and we run
SMC inference on $p(x_{1:T},u_{1:S} | Y) $.

These combination methods are strictly for combining disjoint partitions.  We can
thus use them to combined estimates from the left and right children of discriminant
nodes as per the second term in~\eqref{eq:estimate}. To combine estimates from parents
and their children, we simply note that the weighted sum of two consistent independent
consistent estimators is itself consistent if the weights sum to $1$.  Thus we can view
$\frac{c_j-\left(c_{l_j}+c_{r_j}\right)}{c_j}$ as a parent weight and $\frac{c_{l_j}+c_{r_j}}{c_j}$
as a child weight, which are then used to combine the two independent estimators
in~\eqref{eq:estimate}.

==> discrete.tex <==
% !TEX root =  it_icml2018.tex

ITs can in practice be used for arbitrary parameter spaces $\X_T$
provided the number of variables $T$ is bounded (and even this might be potentially
be relaxed).  There two general approaches we can take when $x_t \notin \real$,
restricting the splits or reparameterizing $x_{1:T}$, which we now consider in turn.

\subsection{Restricting the Splits}

The approach of restricting the splits is
 less general as it requires the number of variables to
remain fixed and imposes additional restrictions, but 
it may be more natural in a number of situations, particularly when each $x_t$ is
discrete.  To illustrate this approach, consider the following simple proposal for
a discrete problem where $\X_T =  \{0,1\}^2$
\begin{align}
q(x_1) &= \begin{cases}
0.75 &\text{if } x_1 = 0 \\
0.25 &\text{if } x_1 = 1
\end{cases} \\
q(x_2 | x_1) &= \begin{cases}
0.8 &\text{if } x_1 = 0, \, x_2 = 0\\
0.1 &\text{if } x_1 = 0, \, x_2 = 1\\
0.4 &\text{if } x_1 = 0, \, x_2 = 0\\
0.6 &\text{if } x_1 = 1, \, x_2 = 1
\end{cases}
\end{align}
and we use the cumulative distribution function mapping considered 
in the main paper.  More precisely, we can exploit the fact that we only
ever need to calculate the inverse mappings and defining these such that drawing
$z_1$ and $z_2$ independently from continuous uniform distributions between $0$
and $1$ and applying the inverse mappings gives the correct distribution 
on $x_1$ and $x_2$.  We can now split $z_1$ and still ensure that any given
$x_{1:2}$ is assigned to a unique child by restricting this split to be at the point
$0.75$, leading to partitions
of $x_1=0$ and $x_2=1$ respectively.  However, if we instead consider splitting
$z_2$, we see that there is no possible split point that gives disjoint partitions on $\X_T$.
For example, if we split at $z_{2} = 0.8$ then $x_{1:2} =  \{1,1\}$ could fall into
either of the generated partitions: $z_{1:2} = \{0.8,0.7\}$ and $z_{1:2} = \{0.8,0.9\}$
both map to $x_{1:2} =  \{1,1\}$, but fall on opposite sides of the split.

Fortunately, there are two clearcut ways of overcoming this problem.  Firstly, instead of
using cumulative distribution functions, we can restrict the $\eta_t (x_t;x_{1:t-1})$
to be functions of only $x_t$, such that each dimension is mapped separately.\footnote{As
per the earlier example, it will generally be necessary to define the inverse of $\eta_t$
directly.}
For purely discrete problems, this is effectively equivalent to doing away with the
mapping entirely and splitting into disjoint sets of outcomes for a particular $x_t$,
akin to how discrete variables are dealt with in decision trees.  Practically, care might still be
required to avoid superfluous splits -- splits higher up the tree might mean that
certain $x_t$ have zero probability -- and it may become more challenging to 
calculate the renormalized density functions for the truncated proposals,
but neither of these threaten the convergence of the algorithm.

Alternatively, and perhaps more practically, we can instead restrict the order of the
splits.  For a given 

